A Systematic Survey on Android API Usage for Data-Driven Analytics with Smartphones

Recent industrial and academic research has focused on data-driven analytics with smartphones by collecting user interaction, context, and device systems data through Application Programming interfaces (APIs) and sensors. The Android OS provides various APIs to collect such mobile usage and sensor data for third-party developers. Usage Statistics API (US API) and Accessibility Service API (AS API) are representative Android APIs for collecting app usage data and are used for various research purposes as they can collect fine-grained interaction data (e.g., app usage history, user interaction type). Furthermore, other sensor APIs help to collect a user's context and device state data, along with AS/US APIs. This review investigates mobile usage and sensor data-driven research using AS/US APIs, by categorizing the research purposes and the data types. In this paper, the surveyed studies are classified as follows: five themes and 21 subthemes, and a four-layer hierarchical data classification structure. This allows us to identify a data usage trend and derive insight into data collection according to research purposes. Several limitations and future research directions of mobile usage and sensor data-driven analytics research are discussed, including the impact of changes in the Android API versions on research, the privacy and data quality issues, and the mitigation of reproducibility risks with standardized data typology.

==> tables/accessibilityevents.tex <==
\begin{table}
\caption{Types of AccessibilityEvent ~\cite{AccessibilityEvent}}
\centering
\begin{adjustbox}{max width=0.8\textwidth}
\tiny{
\begin{tabular}{cl@{\hskip 0.25in}l@{\hskip 0.3in}c}

\toprule

\raisebox{0.5em}{\textbf{Event Types}} & 
\multicolumn{1}{c}{\raisebox{0.5em}{\textbf{Event}}} & 
\multicolumn{1}{c}{\raisebox{0.5em}{\textbf{Event Description}}} & 
\textbf{\shortstack{Added\\ API level}} \\
\hline\hline

\multirow{9}{*}{\shortstack{VIEW\\TYPES}} &
\multirow{1}{*}{\texttt{TYPE\char`_VIEW\char`_CLICKED}} & 
\multirow{1}{*}{\shortstack[l]{``The events of clicking on a View like Button, CompoundButton, etc.''}} & 
\multirow{1}{*}{4} \\

&
\multirow{1}{*}{\texttt{TYPE\char`_VIEW\char`_LONG\char`_CLICKED}} & 
\multirow{1}{*}{\shortstack[l]{``The events of long clicking on a View like Button, CompoundButton, etc''}} & 
\multirow{1}{*}{4} \\

&
\multirow{1}{*}{\texttt{TYPE\char`_VIEW\char`_SELECTED}} & 
\multirow{1}{*}{\shortstack[l]{``The event of selecting an item in context of an AdapterView''}} & 
\multirow{1}{*}{4} \\

&
\multirow{1}{*}{\texttt{TYPE\char`_VIEW\char`_FOCUSED}} & 
\multirow{1}{*}{\shortstack[l]{``The event of setting input focus of a View''}} & 
\multirow{1}{*}{4} \\

&
\multirow{1}{*}{\texttt{TYPE\char`_VIEW\char`_TEXT\char`_CHANGED}} & 
\multirow{1}{*}{\shortstack[l]{``The event of changing the text of an EditText''}} & 
\multirow{1}{*}{4} \\

&
\multirow{1}{*}{\texttt{TYPE\char`_VIEW\char`_TEXT\char`_SELECTION\char`_CHANGED}} & 
\multirow{1}{*}{\shortstack[l]{``The event of changing the selection in an EditText''}} & 
\multirow{1}{*}{14} \\

&
\multirow{1}{*}{\texttt{TYPE\char`_VIEW\char`_TEXT\char`_TRAVERSED\char`_AT\char`_MOVEMENT\char`_GRANULARITY}} & 
\multirow{1}{*}{\shortstack[l]{``The event of traversing the text of a view at a given movement granularity''}} & 
\multirow{1}{*}{16} \\

&
\multirow{1}{*}{\texttt{TYPE\char`_VIEW\char`_SCROLLED}} & 
\multirow{1}{*}{\shortstack[l]{``The event of scrolling a view''}} & 
\multirow{1}{*}{14} \\

&
\multirow{1}{*}{\texttt{TYPE\char`_VIEW\char`_CONTEXT\char`_CLICKED}} & 
\multirow{1}{*}{\shortstack[l]{``The event of a context click on a view''}} & 
\multirow{1}{*}{23} \\
\cmidrule(l){1-4}


\multirow{6}{*}{\shortstack{TRANSITION\\TYPES}} &
\multirow{1}{*}{\texttt{TYPE\char`_WINDOW\_STATE\char`_CHANGED}} & 
\multirow{1}{*}{\shortstack[l]{``The event of change to a visually distinct section of the user interface''}} & 
\multirow{1}{*}{4} \\

&
\multirow{2}{*}{\raisebox{-1em}{\texttt{TYPE\char`_WINDOW\_CONTENT\char`_CHANGED}}} &
\multirow{2}{*}{\raisebox{-2em}{\shortstack[l]{``The event of changing content of a window and\\ more specifically the sub-tree rooted at the event's source''}}} & 
\multirow{2}{*}{\raisebox{-1.5em}{\shortstack{Event: 14\\Sub Event: 19, 28, 30}}} \\
& & & \\

&
\multirow{3}{*}{\texttt{TYPE\char`_WINDOW\char`_CHANGED}} & 
\multirow{3}{*}{\shortstack[l]{``The event change in the system windows shown on the screen''}} & 
\multirow{3}{*}{\shortstack{Event: 21\\Sub Event: 28}} \\
& & & \\

\cmidrule(l){1-4}

\multirow{2}{*}{\shortstack{NOTIFICATION\\TYPES}} &
\multirow{2}{*}{\texttt{TYPE\char`_NOTIFICATION\char`_STATE\char`_CHANGED}} & 
\multirow{2}{*}{\shortstack[l]{``The event showing a notification''}} & 
\multirow{2}{*}{4} \\
& & & \\
\cmidrule(l){1-4}


\multirow{8}{*}{\shortstack{EXPLORATION\\TYPES}} &
\multirow{1}{*}{\texttt{TYPE\char`_VIEW\char`_HOVER\char`_ENTER}} & 
\multirow{1}{*}{\shortstack[l]{``The event of a hover enter over a view''}} & 
\multirow{1}{*}{14} \\


&
\multirow{1}{*}{\texttt{TYPE\char`_VIEW\char`_HOVER\char`_EXIT}} & 
\multirow{1}{*}{\shortstack[l]{``The event of a hover exit over a view''}} & 
\multirow{1}{*}{14} \\


&
\multirow{1}{*}{\texttt{TYPE\char`_TOUCH\char`_INTERACTION\char`_START}} & 
\multirow{1}{*}{\shortstack[l]{``The event of the user starting to touch the screen''}} & 
\multirow{1}{*}{17} \\


&
\multirow{1}{*}{\texttt{TYPE\char`_TOUCH\char`_INTERACTION\char`_END}} & 
\multirow{1}{*}{\shortstack[l]{``The event of the user ending to touch the screen''}} & 
\multirow{1}{*}{17} \\


&
\multirow{1}{*}{\texttt{TYPE\char`_TOUCH\char`_EXPLORATION\char`_GESTURE\char`_START}} & 
\multirow{1}{*}{\shortstack[l]{``The event of starting a touch exploration gesture''}} & 
\multirow{1}{*}{14} \\


&
\multirow{1}{*}{\texttt{TYPE\char`_TOUCH\char`_EXPLORATION\char`_GESTURE\char`_END}} & 
\multirow{1}{*}{\shortstack[l]{``The event of ending a touch exploration gesture''}} & 
\multirow{1}{*}{14} \\


&
\multirow{1}{*}{\texttt{TYPE\char`_GESTURE\char`_DETECTION\char`_START}} & 
\multirow{1}{*}{\shortstack[l]{``The event of beginning gesture detection''}} &
\multirow{1}{*}{17} \\


&
\multirow{1}{*}{\texttt{TYPE\char`_GESTURE\char`_DETECTION\char`_END}} & 
\multirow{1}{*}{\shortstack[l]{``The event of ending gesture detection''}} & 
\multirow{1}{*}{17} \\
\cmidrule(l){1-4}


\multirow{2}{*}{\shortstack{MICELLANEOUS\\TYPES}} &
\multirow{2}{*}{\texttt{TYPE\char`_ANNOUNCEMENT}} & 
\multirow{2}{*}{\shortstack[l]{``The event of an application making an announcement''}} & 
\multirow{2}{*}{16} \\
& & & \\
\cmidrule(l){1-4}


\multirow{5}{*}{\shortstack{ETC}} &
\multirow{1}{*}{\texttt{TYPE\char`_VIEW\char`_ACCESSIBILITY\char`_FOCUS}} & 
\multirow{1}{*}{\shortstack[l]{``The event of gaining accessibility focus''}} &
\multirow{1}{*}{16} \\


& 
\multirow{1}{*}{\texttt{TYPE\char`_VIEW\char`_ACCESSIBILITY\char`_FOCUS\char`_CLEARED}} & 
\multirow{1}{*}{\shortstack[l]{``The event of clearing accessibility focus''}} & 
\multirow{1}{*}{16} \\


& 
\multirow{1}{*}{\texttt{TYPE\char`_ALL\char`_MASK}} & 
\multirow{1}{*}{\shortstack[l]{``Mask for AccessibilityEvent all types''}} & 
\multirow{1}{*}{4} \\


& 
\multirow{1}{*}{\texttt{TYPE\char`_ASSIST\char`_READING\char`_CONTEXT}} & 
\multirow{1}{*}{\shortstack[l]{``The event of the assistant currently reading the users screen context''}} & 
\multirow{1}{*}{23} \\


& 
\multirow{1}{*}{\texttt{INVALID\char`_POSITION}} & 
\multirow{1}{*}{\shortstack[l]{``Invalid selection/focus position''}} & 
\multirow{1}{*}{4} \\



\bottomrule
\end{tabular}}
\end{adjustbox}
\label{table:accessibilityeventtypes}
\end{table}


==> tables/discussion1.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
% \usepackage{multirow}
% \usepackage{graphicx}
% \usepackage[table,xcdraw]{xcolor}
% If you use beamer only pass "xcolor=table" option, i.e. \documentclass[xcolor=table]{beamer}
\begin{table}
\caption{Number of surveyed studies in each research themes and sub-themes via the types of IP criteria}
\label{table:discussion1}
\begin{threeparttable}
\centering
\resizebox{\textwidth}{!}{%
\begin{tabular}{@{}ccrlrlp{3cm}p{3cm}c@{}}
\toprule
 &  & \multicolumn{4}{c}{\textbf{IP1: Studies for People without Disabilities}}                                                                                                 
 & \multicolumn{2}{c}{\textbf{IP2: Studies for People with Disabilities}}                                                              
 & \\ \cmidrule(lr){3-8}
\multirow{-2}{*}{\textbf{Theme}} & \multirow{-2}{*}{\textbf{Sub-Theme}} & \multicolumn{1}{c}{\textbf{IP1-1-AS}}            & \multicolumn{1}{c}{\textbf{IP1-1-US}}                                & \multicolumn{1}{c}{\textbf{IP1-2-AS}}            & \multicolumn{1}{c}{\textbf{IP1-2-US}}                                & \multicolumn{1}{c}{\textbf{IP2-1}}            & \multicolumn{1}{c}{\textbf{IP2-2}}            & \multirow{-2}{*}{\textbf{Overall}} \\ \midrule
UP                               & GUPA                                 & \cellcolor[HTML]{96D3A7}5                        & \multicolumn{1}{r}{\cellcolor[HTML]{7DC991}6}                        & \multicolumn{1}{l}{}                             &                                                                      &                                               &                                               & 11                                 \\
UP                               & MLMS                                 & \cellcolor[HTML]{FCFCFF}1                        & \multicolumn{1}{r}{\cellcolor[HTML]{C9E8D3}3}                        & \cellcolor[HTML]{FCFCFF}1                        &                                                                      &                                               &                                               & 5                                  \\
UP                               & FSD                                  & \cellcolor[HTML]{E3F2E9}2                        &                                                                      & \cellcolor[HTML]{7DC991}6                        &                                                                      &                                               &                                               & 8                                  \\
NT                               & IFN                                  & \cellcolor[HTML]{C9E8D3}3                        & \multicolumn{1}{r}{\cellcolor[HTML]{FCFCFF}1}                        & \multicolumn{1}{l}{}                             &                                                                      &                                               &                                               & 4                                  \\
NT                               & NT/NM                                & \cellcolor[HTML]{7DC991}6                        & \multicolumn{1}{r}{\cellcolor[HTML]{E3F2E9}2}                        & \multicolumn{1}{l}{}                             &                                                                      &                                               &                                               & 8                                  \\
NT                               & HNAU                                 & \cellcolor[HTML]{7DC991}6                        &                                                                      & \multicolumn{1}{l}{}                             &                                                                      &                                               &                                               & 6                                  \\
EUI/UX                           & CE                                   & \cellcolor[HTML]{FCFCFF}1                        &                                                                      & \cellcolor[HTML]{C9E8D3}3                        &                                                                      &                                               &                                               & 4                                  \\
EUI/UX                           & UIE                                  & \cellcolor[HTML]{E3F2E9}2                        &                                                                      & \cellcolor[HTML]{E3F2E9}2\tnote{*} & \multicolumn{1}{r}{\cellcolor[HTML]{FCFCFF}1\tnote{*}} &                                               &                                               & 5                                  \\
EUI/UX                           & UIP                                  & \cellcolor[HTML]{E3F2E9}2                        &                                                                      & \cellcolor[HTML]{FCFCFF}1                        &                                                                      &                                               &                                               & 3                                  \\
EUI/UX                           & IFASD                                & \multicolumn{1}{l}{}                             &                                                                      & \multicolumn{1}{l}{}                             &                                                                      & \multicolumn{1}{r}{\cellcolor[HTML]{63BE7B}7} & \multicolumn{1}{r}{\cellcolor[HTML]{E3F2E9}2} & 9                                  \\
EUI/UX                           & DEASD                                & \multicolumn{1}{l}{}                             &                                                                      & \multicolumn{1}{l}{}                             &                                                                      & \multicolumn{1}{r}{\cellcolor[HTML]{63BE7B}7} & \multicolumn{1}{r}{\cellcolor[HTML]{FCFCFF}1} & 8                                  \\
EUI/UX                           & CFASD                                & \multicolumn{1}{l}{}                             &                                                                      & \multicolumn{1}{l}{}                             &                                                                      & \multicolumn{1}{r}{\cellcolor[HTML]{C9E8D3}3} &                                               & 3             \\                   
PS                               & ASS                                  & \cellcolor[HTML]{C9E8D3}3                        & \multicolumn{1}{r}{\cellcolor[HTML]{C9E8D3}3}                        & \multicolumn{1}{l}{}                             &                                                                      &                                               &                                               & 6                                  \\
PS                               & APC                                  & \cellcolor[HTML]{E3F2E9}2\tnote{*} & \multicolumn{1}{r}{\cellcolor[HTML]{FCFCFF}1\tnote{*}} & \multicolumn{1}{l}{}                             &                                                                      &                                               &                                               & 3                                  \\
PS                               & PPS                                  & \cellcolor[HTML]{C9E8D3}3                        & \multicolumn{1}{r}{\cellcolor[HTML]{FCFCFF}1}                        & \cellcolor[HTML]{FCFCFF}1                        &                                                                      &                                               &                                               & 5                                  \\
PS                               & MDPS                                 & \cellcolor[HTML]{FCFCFF}1                        &                                                                      & \cellcolor[HTML]{96D3A7}5                        & \multicolumn{1}{r}{\cellcolor[HTML]{E3F2E9}2}                        &                                               &                                               & 8                                  \\
PTS                              & GAT                                  & \cellcolor[HTML]{FCFCFF}1                        &                                                                      & \cellcolor[HTML]{C9E8D3}3                        &                                                                      &                                               &                                               & 4                                  \\
PTS                              & CT                                   & \multicolumn{1}{l}{}                             &                                                                      & \cellcolor[HTML]{E3F2E9}2                        &                                                                      &                                               &                                               & 2                                  \\
PTS                              & APS                                  & \cellcolor[HTML]{E3F2E9}2                        &                                                                      & \cellcolor[HTML]{E3F2E9}2                        &                                                                      &                                               &                                               & 4                                  \\
PTS                              & PMM                                  & \cellcolor[HTML]{FCFCFF}1                        & \multicolumn{1}{r}{\cellcolor[HTML]{FCFCFF}1}                        & \multicolumn{1}{l}{}                             &                                                                      &                                               &                                               & 2                                  \\
PTS                              & TRSGT                                & \cellcolor[HTML]{E3F2E9}2                        &                                                                      & \cellcolor[HTML]{E3F2E9}2                        &                                                                      &                                               &                                               & 4                                  \\ \midrule
\multicolumn{2}{c}{Overall}                                             & 43                                               & \multicolumn{1}{r}{18}                                               & 28                                               & \multicolumn{1}{r}{3}                                                & \multicolumn{1}{r}{17}                        & \multicolumn{1}{r}{3}                         & 112-2\tnote{*} = 100                        \\ \bottomrule
\end{tabular}%
}
\begin{tablenotes}
\scriptsize
    \item[*]Bonné et al. [17] and Ryu et al. [131], which is used AS/US APIs both, were included in IP1-1-AS/US and IP1-2-AS/US twice, respectively. \\ Therefore, the number of surveyed studies in this study is 110, excluding the count of two out of a total of 112 overalls.
\end{tablenotes}
\end{threeparttable}
\end{table}

==> tables/discussion2.tex <==
\begin{table}
\caption{Types of data used in surveyed papers according to types of IP}
\centering
\begin{adjustbox}{max width=\textwidth}
\begin{tabular}{c ccccccc c cccccc c ccccccc c cccc}
\toprule

\multirow{14}{*}{\textbf{\begin{tabular}[c]{@{}c@{}}Type of\\Included\\Papers\end{tabular}}} & 
\multicolumn{7}{c}{Interaction sensing} & 
\multirow{14}{*}{} &
\multicolumn{6}{c}{System sensing} &
\multirow{14}{*}{} &
\multicolumn{7}{c}{Context sensing} & 
\multirow{14}{*}{} &
\multirow[b]{14}{*}{\raisebox{1.5em}{\rotatebox{90}{\textbf{\shortstack{\# of types of data categories}}}}} & 
\multirow[b]{14}{*}{\raisebox{1.5em}{\rotatebox{90}{\textbf{\shortstack{Sum of utilized data categories}}}}} & 
\multirow[b]{14}{*}{\raisebox{1.5em}{\rotatebox{90}{\textbf{\shortstack{\# of surveyed studies}}}}} &
\multirow[b]{14}{*}{\raisebox{1.5em}{\rotatebox{90}{\textbf{\shortstack{Average of data categories \\ \hspace{-0.8em} used per surveyed study}}}}} \\
\cmidrule(l){2-8} \cmidrule(l){10-15} \cmidrule(l){17-23}

& 
\multirow[b]{13}{*}{\raisebox{2em}{\rotatebox{90}{\textbf{App usage patterns}}}} &
\multicolumn{4}{c}{User Interaction} &
\multirow[b]{13}{*}{\raisebox{2em}{\rotatebox{90}{\textbf{Notifications}}}} &
\multirow[b]{13}{*}{\raisebox{2em}{\rotatebox{90}{\textbf{Contacts information}}}} & &

\multirow[b]{13}{*}{\raisebox{2em}{\rotatebox{90}{\textbf{Calendar and Standard Time}}}} &
\multirow[b]{13}{*}{\raisebox{2em}{\rotatebox{90}{\textbf{Device setting}}}} &
\multirow[b]{13}{*}{\raisebox{2em}{\rotatebox{90}{\textbf{Device sound states}}}} &
\multirow[b]{13}{*}{\raisebox{2em}{\rotatebox{90}{\textbf{Device Battery states}}}} &
\multirow[b]{13}{*}{\raisebox{2em}{\rotatebox{90}{\textbf{Device Operation states}}}} &
\multirow[b]{13}{*}{\raisebox{2em}{\rotatebox{90}{\textbf{Device screen states}}}} & &

\multirow[b]{13}{*}{\raisebox{2em}{\rotatebox{90}{\textbf{Microphone}}}} &
\multirow[b]{13}{*}{\raisebox{2em}{\rotatebox{90}{\textbf{Light}}}} &
\multirow[b]{13}{*}{\raisebox{2em}{\rotatebox{90}{\textbf{Motion}}}} &
\multirow[b]{13}{*}{\raisebox{2em}{\rotatebox{90}{\textbf{Proximity}}}} &
\multirow[b]{13}{*}{\raisebox{2em}{\rotatebox{90}{\textbf{Network information}}}} &
\multirow[b]{13}{*}{\raisebox{2em}{\rotatebox{90}{\textbf{GPS}}}} &
\multirow[b]{13}{*}{\raisebox{2em}{\rotatebox{90}{\textbf{Camera}}}} & & 
& & & \\
\cmidrule(l){3-6}

&
&
\multirow[b]{12}{*}{\raisebox{2.5em}{\rotatebox{90}{\textbf{Type of Interaction}}}} &
\multirow[b]{12}{*}{\raisebox{2.5em}{\rotatebox{90}{\textbf{UI changed}}}} &
\multirow[b]{12}{*}{\raisebox{2.5em}{\rotatebox{90}{\textbf{Time of Interaction}}}} &
\multirow[b]{12}{*}{\raisebox{2.5em}{\rotatebox{90}{\textbf{Target of Interaction}}}} &
& & &
& & & & & & &
& & & & & & & &
& & &  \\

& & & & & & & & & & & & & & & & & & & & & & & & & & & \\
& & & & & & & & & & & & & & & & & & & & & & & & & & & \\
& & & & & & & & & & & & & & & & & & & & & & & & & & & \\
& & & & & & & & & & & & & & & & & & & & & & & & & & & \\
& & & & & & & & & & & & & & & & & & & & & & & & & & & \\
& & & & & & & & & & & & & & & & & & & & & & & & & & & \\
& & & & & & & & & & & & & & & & & & & & & & & & & & & \\
& & & & & & & & & & & & & & & & & & & & & & & & & & & \\
& & & & & & & & & & & & & & & & & & & & & & & & & & & \\

\hline\hline

IP1-1-AS & \cellcolor[HTML]{63BE7B}23 & \cellcolor[HTML]{71C487}21 & \cellcolor[HTML]{ADDCBB}12 & \cellcolor[HTML]{E2F2E9}4  & \cellcolor[HTML]{9FD7AF}14 & \cellcolor[HTML]{71C487}21 & \cellcolor[HTML]{CEEAD7}7 & & \cellcolor[HTML]{E2F2E9}4  &  & \cellcolor[HTML]{BAE2C6}10  & \cellcolor[HTML]{CEEAD7}7 & \cellcolor[HTML]{DBEFE3}5 & \cellcolor[HTML]{9FD7AF}14 & & \cellcolor[HTML]{E9F4EE}3& \cellcolor[HTML]{E2F2E9}4 & \cellcolor[HTML]{A6D9B5}13 & \cellcolor[HTML]{E9F4EE}3 & \cellcolor[HTML]{A6D9B5}13 & \cellcolor[HTML]{B3DFC0}11  & \cellcolor[HTML]{EFF7F4}2 & &   \cellcolor[HTML]{F8696B}20 & \cellcolor[HTML]{FAAAAC}191 & \cellcolor[HTML]{FBBDC0}43 & \cellcolor[HTML]{F8696B}4.4 \\

IP1-1-US & \cellcolor[HTML]{8BCF9E}17 & \cellcolor[HTML]{EFF7F4}2  & \multicolumn{1}{l}{}       & \multicolumn{1}{l}{}       & \multicolumn{1}{l}{}       & \multicolumn{1}{r}{\cellcolor[HTML]{E9F4EE}3}  & \cellcolor[HTML]{F6FAFA}1  & & \cellcolor[HTML]{F6FAFA}1 &   &   & &  \cellcolor[HTML]{F6FAFA}1 & \cellcolor[HTML]{D5ECDD}6 &   &   & & \cellcolor[HTML]{D5ECDD}6 & \multicolumn{1}{r}{\cellcolor[HTML]{EFF7F4}2} &         & \cellcolor[HTML]{E2F2E9}4  &   & & \cellcolor[HTML]{FBB7B9}10 & \cellcolor[HTML]{FCEBED}43  & \cellcolor[HTML]{FCE5E8}17 & \cellcolor[HTML]{FBBBBE}2.5 \\

IP1-2-AS & \cellcolor[HTML]{D5ECDD}6  & \cellcolor[HTML]{77C78D}20 & \cellcolor[HTML]{DBEFE3}5  & \cellcolor[HTML]{E9F4EE}3  & \cellcolor[HTML]{77C78D}20 &                                                & \cellcolor[HTML]{E9F4EE}3 & & \cellcolor[HTML]{E9F4EE}3 & \multicolumn{1}{r}{\cellcolor[HTML]{F6FAFA}1} & \multicolumn{1}{r}{\cellcolor[HTML]{EFF7F4}2}  & \multicolumn{1}{r}{\cellcolor[HTML]{EFF7F4}2} & \cellcolor[HTML]{F6FAFA}1 & \cellcolor[HTML]{F6FAFA}1 & & \multicolumn{1}{r}{\cellcolor[HTML]{EFF7F4}2} & \multicolumn{1}{r}{\cellcolor[HTML]{E9F4EE}3} & \cellcolor[HTML]{E2F2E9}4  &                                               & \cellcolor[HTML]{E9F4EE}3  & \cellcolor[HTML]{E2F2E9}4  & \multicolumn{1}{r}{\cellcolor[HTML]{F6FAFA}1} & & \cellcolor[HTML]{F9797B}18 & \cellcolor[HTML]{FCD9DB}84  & \cellcolor[HTML]{FBD6D9}27 & \cellcolor[HTML]{FAA2A5}3.1 \\

IP1-2-US & 
\cellcolor[HTML]{EFF7F4}2 & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & &
\multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} &  &
\multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & &
\cellcolor[HTML]{FCFCFF}1  & \cellcolor[HTML]{FCFCFF}2 & \cellcolor[HTML]{FCFCFF}2  & \cellcolor[HTML]{FCFCFF}1.0\\

IP2-1 & 
\cellcolor[HTML]{EFF7F4}2 & \cellcolor[HTML]{E9F4EE}3 & \cellcolor[HTML]{F6FAFA}1  & \cellcolor[HTML]{E9F4EE}3 & \cellcolor[HTML]{CEEAD7}7 &  &  & &
 &  &  &  &  &  &  &
 &  & \cellcolor[HTML]{F6FAFA}1 & & \cellcolor[HTML]{F6FAFA}1 & \cellcolor[HTML]{F6FAFA}1 &  & & \cellcolor[HTML]{FBC6C9}8 & \cellcolor[HTML]{FCF5F8}19 & \cellcolor[HTML]{FCF3F6}8 & \cellcolor[HTML]{FBC2C4}2.4 \\

sum & 
\cellcolor[HTML]{63BE7B}50 & \cellcolor[HTML]{70C486}46 & \cellcolor[HTML]{C7E7D2}18 & \cellcolor[HTML]{E0F1E7}10 & \cellcolor[HTML]{80CA94}41 & \cellcolor[HTML]{B5DFC2}24 & \cellcolor[HTML]{DDF0E5}11 & &
\cellcolor[HTML]{E7F4ED}8 & \multicolumn{1}{r}{\cellcolor[HTML]{FCFCFF}1} & \multicolumn{1}{r}{\cellcolor[HTML]{DAEFE2}12} & \multicolumn{1}{r}{\cellcolor[HTML]{E4F2EA}9} & \cellcolor[HTML]{EAF5EF}7 & \cellcolor[HTML]{BEE3CA}21 & & \multicolumn{1}{r}{\cellcolor[HTML]{F0F7F5}5} & \multicolumn{1}{r}{\cellcolor[HTML]{EAF5EF}7} & \cellcolor[HTML]{B5DFC2}24 & \multicolumn{1}{r}{\cellcolor[HTML]{F0F7F5}5} & \cellcolor[HTML]{CBE8D4}17 & \cellcolor[HTML]{C1E4CC}20 & \multicolumn{1}{r}{\cellcolor[HTML]{F6FAFA}3} & &
\cellcolor[HTML]{F8696B}20 & \cellcolor[HTML]{F8696B}339 & \cellcolor[HTML]{F8696B}97 & \cellcolor[HTML]{FA9294}3.5\\

\bottomrule
\end{tabular}
\label{table:discussion2}
\end{adjustbox}
\end{table}


==> tables/existingreviewstudies.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
% \usepackage{graphicx}
\begin{table}[]
\caption{List of existing studies that investigated prior work that employed mobile usage and sensor data}
\resizebox{\textwidth}{!}{%
\begin{tabular}{@{}lclll@{}}
\toprule
\multicolumn{1}{c}{\textbf{Ref.}}                                & \textbf{\begin{tabular}[c]{@{}c@{}}\ Number of Surveyed \\ Studies\end{tabular}} & \multicolumn{1}{c}{\textbf{Purpose of Review}}                                                                                                                    & \multicolumn{1}{c}{\textbf{Reviewed Items}}                                                 & \multicolumn{1}{c}{\textbf{Type of Investigated Data}}                                    \\ \midrule\midrule
Church et al. ~\cite{church2015understanding} & 22                                                                         & \begin{tabular}[c]{@{}l@{}}Review the papers to gain a more generalizable \\ understanding of mobile device use across \\ different user populations\end{tabular} & \begin{tabular}[c]{@{}l@{}}Number of participants, experiment duration, \\ deployment, recruitment, incentives, method, \\ data collected, user input\end{tabular}                                                                          & \begin{tabular}[c]{@{}l@{}}Time, communication, mobility, battery, screen, \\ notifications, multimedia, applications, locations, touch\end{tabular}                      \\ \midrule
Rooksby et al. ~\cite{rooksby2019student} & 19                                              & \begin{tabular}[c]{@{}l@{}}Review the papers using sensor data for \\ monitoring student mental health\end{tabular}                                               & \begin{tabular}[c]{@{}l@{}}Utilized data, experiment duration, \\ number of participants\end{tabular}                                                                                                                                                               & \begin{tabular}[c]{@{}l@{}}Acceleration, activity, app usage, battery, charge, \\ browser history, Bluetooth, call logs, camera events, \\ screen, keyboard, UI, location, light sensor, microphone, \\ SMS/email\end{tabular}                                                                                                                                          \\ \midrule
Kortis et al. ~\cite{kourtis2019digital} & 62                                                                         & \begin{tabular}[c]{@{}l@{}}Review the papers using mobile and \\ wearable device data for tracking \\ the digital biomarker for Alzheimer's disease\end{tabular}  & Utilized data, sense domain, metrics                                                                                                                             & \begin{tabular}[c]{@{}l@{}}Camera, microphone, acceleration/gyro, barometer, \\ touchscreen, geoposition, device use, ECG, PPG, \\ IR thermometer, ballistocardiography, galvanic skin response, \\ ambient light sensor, UV sensor, electromyogram (EMG)\end{tabular}                                                                                                                                                                      \\ \midrule
Berkel et al. ~\cite{van2017experience} & 110                                               & \begin{tabular}[c]{@{}l@{}}Review the papers using experience \\ sampling method (ESM) on mobile devices\end{tabular}                                             
& \begin{tabular}[c]{@{}l@{}}Experiment duration, trigger, response rate, \\ compensate, personal device, utilized data\end{tabular}                                                                                                                                             & \begin{tabular}[c]{@{}l@{}}ESM, location, phone calls, network related, bio-signal (s), \\ accelerometer, app usage, other (s)\end{tabular}                                                                                                                                        \\ \midrule
Liang et al. ~\cite{liang2019survey} 
& \begin{tabular}[c]{@{}c@{}}approximately \\ 92\end{tabular}                
& \begin{tabular}[c]{@{}l@{}}Review the papers using various data \\ including smartphone data \\ in digital phenotyping for mental health\end{tabular}             & \begin{tabular}[c]{@{}l@{}} \tabitem Data collection strategies \\ (data, strategy, pros, cons)\\ \tabitem List of affect lexicons \\ (category, lexicon, affect type, vocabulary)\\ \tabitem Applications for mental health \\(type, name, symptom, data)\\ \tabitem Affect recognition \\ (modality, category, work, algorithm) \\ \tabitem Behavior anomaly detection \\(category, sensor, work, algorithm)\end{tabular} & \begin{tabular}[c]{@{}l@{}} \tabitem Physical data: facial expressions, behavioral data, \\ vocal data, context data (e.g., location, timestamp)\\ \tabitem Cyber data: online behaviors, social media data\\ \tabitem Biological data: blood oxygen saturation, blood pressure, \\ heartbeat rate, respiration frequency, brain waves \\ \tabitem Social data: call logs, text messages, GPS location, \\ hot spots, email, friendship list, online activities \\ (e.g., like, comment, sharing)\end{tabular} \\ \bottomrule


\end{tabular}%
\label{table:existingresearch}
}
\end{table}

==> tables/history.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% \usepackage{graphicx}
% \usepackage[table,xcdraw]{xcolor}
% If you use beamer only pass "xcolor=table" option, i.e. \documentclass[xcolor=table]{beamer}
\begin{table}[]
\centering
\caption{Impact on research theme and sub-theme according to API change history}
\label{table:history}
\resizebox{\textwidth}{!}{%
\begin{tabular}{@{}rrll|llllll|lll|lll|llll|lllll@{}}
\toprule
\multicolumn{1}{c}{} &
  \multicolumn{1}{c}{} &
  \multicolumn{1}{c}{} &
  \multicolumn{1}{c|}{} &
  \multicolumn{6}{c|}{\textbf{EUI/UX}} &
  \multicolumn{3}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{UP}} &
  \multicolumn{3}{c|}{\textbf{NT}} &
  \multicolumn{4}{c|}{\textbf{PS}} &
  \multicolumn{5}{c}{\textbf{PTS}} \\ \cmidrule(l){5-25} 
\multicolumn{1}{c}{\multirow{-2}{*}{Year}} &
  \multicolumn{1}{c}{\multirow{-2}{*}{API Level}} &
  \multicolumn{1}{c}{\multirow{-2}{*}{Published API}} &
  \multicolumn{1}{c|}{\multirow{-2}{*}{Updated API}} &
  \multicolumn{1}{c}{\textbf{CE}} &
  \multicolumn{1}{c}{\textbf{UIE}} &
  \multicolumn{1}{c}{\textbf{UIP}} &
  \multicolumn{1}{c}{\textbf{IFASD}} &
  \multicolumn{1}{c}{\textbf{DEASD}} &
  \multicolumn{1}{c|}{\textbf{CFASD}} &
  \multicolumn{1}{c}{\textbf{GUPA}} &
  \multicolumn{1}{c}{\textbf{MLMS}} &
  \multicolumn{1}{c|}{\textbf{FSD}} &
  \multicolumn{1}{c}{\textbf{IFN}} &
  \multicolumn{1}{c}{\textbf{NT/NM}} &
  \multicolumn{1}{c|}{\textbf{HNAU}} &
  \multicolumn{1}{c}{\textbf{ASS}} &
  \multicolumn{1}{c}{\textbf{APC}} &
  \multicolumn{1}{c}{\textbf{PPS}} &
  \multicolumn{1}{c|}{\textbf{MDPS}} &
  \multicolumn{1}{c}{\textbf{GAT}} &
  \multicolumn{1}{c}{\textbf{CT}} &
  \multicolumn{1}{c}{\textbf{APS}} &
  \multicolumn{1}{c}{\textbf{PMM}} &
  \multicolumn{1}{c}{\textbf{TRSGT}} \\ \midrule\midrule
2008 &
  1 &
  NotificationManager &
   &
   &
   &
   &
   &
   &
   &
   &
   &
   &
   &
   &
   &
   &
   &
   &
   &
   &
   &
   &
   &
   \\
2009 &
  2$\sim$6 &
  AS API &
   &
   &
   &
   &
   &
   &
   &
   &
   &
   &
   &
   &
   &
   &
   &
   &
   &
   &
   &
   &
   &
   \\
2011 &
  10$\sim$15 &
   &
  AS API &
   &
   &
   &
   &
   &
   &
   &
   &
   &
   &
   &
   &
   &
   &
   &
   &
   &
   &
   &
   &
   \\
2012 &
  16$\sim$17 &
   &
  AS API &
   &
   &
   &
   &
   &
   &
   &
   &
   &
   &
   &
   &
   &
   &
   &
   &
   &
   &
   &
   &
   \\
2013 &
  18$\sim$19 &
  NotificationListenerService &
  AS API &
   &
   &
   &
   &
  \cite{hann2013best} &
   &
   &
   &
   &
   &
   &
   &
   &
   &
   &
   &
   &
   &
   &
   &
   \\
2014 &
  20$\sim$21 &
  US API &
  \begin{tabular}[c]{@{}l@{}}AS API, \\ NotificationListenerService\end{tabular} &
   &
   &
   &
  \cite{zhong2014justspeak} &
  \cite{ganz2014percept} &
   &
  \cite{blanke2014mining, ferreira2014contextual, lee2014hooked} &
   &
  \cite{schweizer2014krakenb, schweizer2014krakena} &
  \cite{pielot2014didn} &
   &
  \cite{pielot2014situ} &
   &
   &
   &
   &
   &
   &
   &
   &
   \\
2015 &
  22$\sim$23 &
   &
  \begin{tabular}[c]{@{}l@{}}NotificationListenerService, \\ NotificationManager\end{tabular} &
   &
   &
  \cite{riegler2015ui} &
  \cite{rodrigues2015breaking, zhong2015enhancing} &
   &
  \cite{rodrigues2015getting} &
  \cite{church2015understanding} &
   &
  \cite{bitsch2015psychologist, ferreira2015aware, montague2015tinyblackbox} &
  \cite{chang2015investigating} &
  \cite{okoshi2015attelia} &
   &
   &
   &
  \cite{ozcan2015babelcrypt} &
   &
   &
   &
   &
   &
   \\
2016 &
  24$\sim$25 &
   &
  \begin{tabular}[c]{@{}l@{}}NotificationListenerService, \\ NotificationManager\end{tabular} &
   &
   &
   &
   &
  \cite{ghidini2016developing} &
  \cite{dobosz2016control} &
  \cite{arruda2016capture, welke2016differentiating, san2016gui} &
  \cite{dutta2016introducing} &
  \cite{andone2016menthal} &
   &
  \cite{okoshi2016towards} &
   &
  \cite{canfora2016silent} &
   &
   &
   &
   &
   &
   &
   & \\
2017 &
  26$\sim$27 &
   &
  NotificationListenerService &
   &
  \cite{zhang2017interaction, ryu2017siginterface} &
   &
  \cite{zhang2017interaction, chinchole2017artificial} &
  \cite{alnfiai2017brailletap} &
   & \cite{singh2017usage}
   &
  \cite{zheng2017cleaning, holzmann2017android} &
   &
   &
  \cite{park2017don, pielot2017beyond, pradhan2017understanding} &
  \cite{chang2017smartphone, dingler2017language, komuro2017relationship}
   &
   &
  \cite{bonne2017exploring} &
   &
   &
  \cite{muangsiri2017random} &
  \cite{wu2017appcheck} &
  \cite{li2017programming, li2017sugilite} &
   &
  \cite{fazzini2017barista, liu2017mechanism} \\
2018 &
  28 &
   &
  AS/US API &
  \cite{sun2018lip, elazhary2018w, tarakji2018voice, wang2018client} &
  \cite{li2018appinite, rauen2018empowering} &
  \cite{riegler2018measuring} &
  \cite{de2018application, rodrigues2018aidme, trindade2018hybrid, zhang2018robust} &
  \cite{chen2018construction, correa2018development} &
   &
  \cite{qin2018deciphering} &
  \cite{lee2018click} &
   &
   &
  \cite{lee2018exploring, lee2018reducing} &
   &
   &
  \cite{rahman2018iac} &
   &
  \cite{li2018chatting, shao2018understanding} &
   &
  \cite{lian2018cat} &
  \cite{li2018kite} &
  \cite{bissig2018towards} &
   \\
2019 &
  29 &
   &
  NotificationManager &
   &
  \cite{chen2019messageontap} &
  \cite{lin2019user} &
   &
  \cite{pareddy2019x, samonte2019braille3d} &
   &
  \cite{kim2019understanding, qin2019association, yuan2019much} &
  \cite{yu2019understanding, yan2019bridging} &
   &
  \cite{visuri2019understanding} &
  \cite{lee2019pass} &
  \cite{lee2019does, anderson2019impact} &
  \cite{aras2019multilock, torres2019behavioral, zhu2019riskcog} &
   &
   &
  \cite{naseri2019accessileaks, wang2019dcdroid} &
  \cite{gu2019practical} &
   &
   &
   &\cite{negara2019practical}
   \\
2020 &
  30 &
   &
  \begin{tabular}[c]{@{}l@{}}AS API, \\ NotificationManager\end{tabular} &
   &
   &
   &
   &
   &
  \cite{alshayban2020accessibility} &
  \cite{radesky2020young}
   &
  \cite{khan2020personal} &
   &
   &
   &
   &
  \cite{zhu2020hybrid} &
   &
  \cite{andriotis2020allow} &
  \cite{leguesse2020reducing, wang2020identifying} &
   &
   &
  \cite{li2020interactive} &
  \cite{xiang2020dynamical} & \\
  \bottomrule
  
\end{tabular}%
}
\end{table}

==> tables/usagestats.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
% \usepackage{multirow}
% \usepackage{graphicx}
\begin{table}[]
\caption{Constants of UsageStatsManager ~\cite{UsageStatsManager} and Events of UsageEvents.Events ~\cite{UsageEvents.Event}}
\resizebox{0.9\textwidth}{!}{%
\begin{tabular}{@{}cllc@{}}
\toprule
\textbf{Class}                             & \multicolumn{1}{c}{\textbf{Constants and Events}} & \multicolumn{1}{c}{\textbf{Description}}                                                                                      & \textbf{\begin{tabular}[c]{@{}c@{}}Android \\ API Level\end{tabular}} \\ \midrule\midrule
\multirow{10}{*}{\textbf{UsageStatsManager}} & INTERVAL\_BEST                                    & "An interval type that will use the best fit interval for the given time range."                                              & 21                                                                    \\ \cmidrule(l){2-4} 
                                             & INTERVAL\_DAILY                                   & "An interval type that spans a day."                                                                                          & 21                    \\ \cmidrule(l){2-4} & INTERVAL\_MONTHLY  
                                             & "An interval type that spans a month."                                                                                        & 21                     \\ \cmidrule(l){2-4} 
                                             & INTERVAL\_WEEKLY                                  & "An interval type that spans a week."                                                                                         & 21                    \\ \cmidrule(l){2-4} 
                                             & INTERVAL\_YEARLY                                  & "An interval type that spans a year."                                                                                         & 21                    \\ \cmidrule(l){2-4} 
                                             & STANDBY\_BUCKET\_ACTIVE                           & "The app was used very recently, currently in use or likely to be used very soon."                                            & 28                                                                    \\ \cmidrule(l){2-4} 
                                             & STANDBY\_BUCKET\_FREQUENT                         & "The app was used in the last few days and/ or likely to be used in the next few days."                                       & 28                   \\ \cmidrule(l){2-4} 
                                             & STANDBY\_BUCKET\_RARE                             & "The app has not be used for several days and/or is unlikely to be used for several days."                                    & 28                     \\ \cmidrule(l){2-4} 
                                             & STANDBY\_BUCKET\_RESTRICTED                       & "The app has not be used for several days, is unlikely to be used for several days, and has been misbehaving in some manner." & 30                                                                    \\ \cmidrule(l){2-4} 
                                             & STANDBY\_BUCKET\_WORKING\_SET                     & "The app was used recently and/or likely to be used in the next few hours."                                                   & 28                   \\ \midrule
\multirow{18}{*}{\textbf{UsageEvents.Event}} & ACTIVITY\_PAUSED                                  & "An event type denoting that an Activity moved to the background"                                                             & 29                                                                    \\ \cmidrule(l){2-4} 
                                             & ACTIVITY\_RESUMED                                 & "An event type denoting that an Activity moved to the foreground"                                                             & 29                   \\ \cmidrule(l){2-4} 
                                             & ACTIVITY\_STOPPED                                 & "An activity becomes invisible on the UI, corresponding to Activity.onStop() of the activity's lifecycle"                     & 29                                                        \\ \cmidrule(l){2-4} 
                                             & CONFIGURATION\_CHANGE                             & "An event type denoting that the device configuration has changed."                                                           & 21                                                               \\ \cmidrule(l){2-4} 
                                             & DEVICE\_SHUTDOWN                                  & "An event type denoting that the Android runtime underwent a shutdown process."                                               & 29                     \\ \cmidrule(l){2-4} 
                                             & DEVICE\_STARTUP                                   & "An event type denoting that the Android runtime started up."                                                                 & 29                     \\ \cmidrule(l){2-4} 
                                             & FOREGROUND\_SERVICE\_START                        & "An event type denoting start of a foreground service."                                                                       & 29                                                                    \\ \cmidrule(l){2-4} 
                                             & FOREGROUND\_SERVICE\_STOP                         & "An event type denoting stop of a foreground service."                                                                        & 29                                                                    \\ \cmidrule(l){2-4} 
                                             & KEYGUARD\_HIDDEN                                  & "An event type denoting that the screen's keyguard has been hidden."                                                          & 28                                                                    \\ \cmidrule(l){2-4} 
                                             & KEYGUARD\_SHOWN                                   & "An event type denoting that the screen's keyguard has been shown, whether or not the screen is off."                         & 28                                                                    \\ \cmidrule(l){2-4} 
                                             & MOVE\_TO\_BACKGROUND                              & "This constant was deprecated in API level 29. by ACTIVITY\_PAUSED"                                                           & 21                   \\ \cmidrule(l){2-4} 
                                             & MOVE\_TO\_FOREGROUND                              & "This constant was deprecated in API level 29. by ACTIVITY\_RESUMED"                                                          & 21                   \\ \cmidrule(l){2-4} 
                                             & NONE                                              & "No event type."                                                                                                              & 21                    \\ \cmidrule(l){2-4} 
                                             & SCREEN\_INTERACTIVE                               & "An event type denoting that the screen has gone into an interactive state."                                                  & 28                     \\ \cmidrule(l){2-4} 
                                             & SCREEN\_NON\_INTERACTIVE                          & "An event type denoting that the screen has gone into a non-interactive state."                                               & 28                     \\ \cmidrule(l){2-4} 
                                             & SHORTCUT\_INVOCATION                              & An event type denoting that an action equivalent to a ShortcutInfo is taken by the user.                                      & 25                     \\ \cmidrule(l){2-4} 
                                             & STANDBY\_BUCKET\_CHANGED                          & An event type denoting a change in App Standby Bucket.                                                                        & 28                   \\ \cmidrule(l){2-4} 
                                             & USER\_INTERACTION                                 & An event type denoting that a package was interacted with in some way by the user.                                            & 23                                                                    \\ \bottomrule
\end{tabular}%
\label{table:usagestats}
}
\end{table}
